Precision QCD with the Electron-Ion Collider

This document summarizes the discussions at the program "Precision QCD with the Electron Ion Collider", held from May to June 2025 at the Institute for Nuclear Theory (INT) at the University of Washington. The program was co-sponsored by the INT and by the Center for Frontiers in Nuclear Science (CFNS, Stony Brook University). Over its five-week duration it brought together about 70 theorists, experimentalists and computer scientists all interested in the physics program at the future Electron Ion Collider in preparation at Brookhaven National Laboratory. Key topics at the program were: higher-order perturbative-QCD calculations and techniques; nuclear structure and tomography; comparisons of phenomenological and lattice determinations of parton distribution functions; identification of signature observables for saturated gluons; assessment of the importance of AI techniques for EIC studies and detector development.

==> zz <==

> 
> %commenting out VW original notes
> \iffalse 
> \subsection{TMD global analysis and lattice (Avkhadiev, Bertone, Cerutti, Gamberg, Engelhardt, Prokudin)}
> \noindent
> -- factorization. Status and next-to-leading power\\
> -- need benchmarking of TMD global analysis codes\\
> -- partly in progress, partly done for LHC\\
> -- now have powerful NN techniques\\
> -- dependence on choice for collinear PDFs\\
> -- need to address matching issue. Generally an open issue in TMD physics\\
> -- size of $Y$ term, infer from explicit NNLO calculations. Probably small \\
> -- promote term ``truncation uncertainty" for higher-order uncertainty\\
> -- need NNLL and beyond: NLL would not work for the very precise LHC data\\
> -- CS kernel on lattice:  currently only ASWZ is ``usable", all others are more exploratory. Used in MAP via reweighting \\
> -- twist-3 TMDs on lattice as easy as twist-2\\
> -- role of $b^*$. Particular choice influences extracted result for CS kernel. But how to compare to lattice then? Or conversely, can we really just adopt lattice kernel?\\
> -- related: value of $b_{\mathrm{max}}$\\
> -- $1/b$ corrections? Little known\\
> -- flavor dependence. Needed for HERMES \\
> -- SIDIS normalization issue\\
> -- {\bf for EIC predictions we often don't use the full spread of available analyses. This may give the wrong impression that we already know everything quite precisely (and hence downplay power of EIC). Should always show the full ensemble of predicitions.}
> 
> \subsection{TMD fragmentation (Seidl)}
> Concerning TMD fragmentation functions, FFs, we have now measurements of TMD FFs from $e^+e^-$ annihilation at the Belle experiment \cite{Belle:2019ywy} for pions, kaons and protons relative to the event-shape variable thrust. This data has already been used successfully in a fit \cite{Boglione:2023duo}, but the use of the event shape variables complicates the theoretical interpretation somewhat. From the theoretical side, the measurement of nearly back-to-back hadrons would simplify the description in terms of transverse momentum dependent fragmentation functions only. This has already been analyzed at Belle, but due to the transition from Belle to Belle 2, its publication is significantly delayed and likely requires the inclusion of Belle 2 data before being allowed to proceed. 
> At the same time, for polarized TMD fragmentation, Collins type asymmetries, also using nearly back-to-back hadron pairs have been extracted from Belle \cite{Belle:2019nve,Belle:2008fdv}, Babar \cite{BaBar:2015mcn,BaBar:2013jdt}, and BesIII \cite{BESIII:2015fyw} for mostly charged pions, but also some neutral meson and kaon results are available. At present most of the measurements are projections on typically momentum fractions or transverse momenta, but not yet entirely multidimensional extractions. Those are expected to be added, eventually. 
> Other particle types, especially the Collins FFs for vector mesons which should exhibit an opposite sign according to the Artru model \cite{Artru:1989zv} have so far not been measured. 
> Polarizing TMD FFs are also accessible for $\Lambda$ mesons, but a better understanding of the flavor contributions is still necessary. 
> Collinear fragmentation function measurements, that are the baseline for all TMD FFs, are available for a large number of final states such as light hadrons, various D mesons and even several strongly or weakly decaying lighter mesons \cite{Belle:2024vua}. 
> 
> On the phenomenological side, there is still a substantial discrepancy of the precision of fragmentation function extractions. While collinear, unpolarized FFs are typically known at NNLO, TMD FFs are generally know only to lower orders. In the unpolarized case that N2LL has been reached in global DY, SIDIS and +e+e- fits, but polarized TMD FFs are still only available at leading order. 
> 
> \subsection{Jets and their substructure at EIC  (Arratia, Kang, Lajoie)}
> 
> -- forward-proton direction: ``traditional jets".
> backward: ``small" jets, few hadrons\\
> -- traditionally, cross section presented as function of $p_T$. Better use $Q$? And $x$? \\
> -- need to put theory curves on projected data\\
> -- for future: set standard for how to present data. E.g., state corrections involved \\
> -- small-R jet not DGLAP (beyond NLO) \\
> -- discuss Breit vs Lab frames\\
> -- Centauro jet algorithm for Breit frame\\
> -- need to investigate low and high Q2 regions, both for inclusive jets and when electron is detected.
> -- unqiue role of EECs @ EIC for example q/g tagging.
> 
> \subsection{GPDs at EIC and global analysis (Guo, Hatta, Liuti, Nadel-Turonski, Schönleber)}
> 
> -- overall, large HO corrections. Need to develop for EIC\\
> -- gluon GPDs and exclusive $J/\psi$\\
> -- role of second detector\\
> -- need benchmarking of GPD codes\\
> -- shadow GPDs. Exist also in moment-space (GUMP)?
> Alleviated by using DVMP? \\
> -- twist-3 GPDs still a long way \ldots \\
> -- use lattice?\\
> -- factorization at large $t$, a difficult problem\\
> -- phenomenological relevance?\\
> -- gravitational form factors without gravity. DVCS: impossible inverse problem\ldots \\
> -- $J\psi$ at threshold: better, still tricky\\
> -- better replace ``gravitational" by "mechanical"?
> (stress/forces/pressure). Better suited for communication with other fields
> 
> \fi

